OCC-VO: Dense Mapping via 3D Occupancy-Based Visual Odometry for Autonomous Driving

Visual Odometry (VO) plays a pivotal role in autonomous systems, with a principal challenge being the lack of depth information in camera images. This paper introduces OCC-VO, a novel framework that capitalizes on recent advances in deep learning to transform 2D camera images into 3D semantic occupancy, thereby circumventing the traditional need for concurrent estimation of ego poses and landmark locations. Within this framework, we utilize the TPV-Former to convert surround view cameras' images into 3D semantic occupancy. Addressing the challenges presented by this transformation, we have specifically tailored a pose estimation and mapping algorithm that incorporates Semantic Label Filter, Dynamic Object Filter, and finally, utilizes Voxel PFilter for maintaining a consistent global semantic map. Evaluations on the Occ3D-nuScenes not only showcase a 20.6% improvement in Success Ratio and a 29.6% enhancement in trajectory accuracy against ORB-SLAM3, but also emphasize our ability to construct a comprehensive map. Our implementation is open-sourced and available at: https://github.com/USTCLH/OCC-VO.

==> references_backups <==
@article{mur2017orb,
  title={Orb-slam2: An open-source slam system for monocular, stereo, and rgb-d cameras},
  author={Mur-Artal, Raul and Tard{\'o}s, Juan D},
  journal={IEEE transactions on robotics},
  volume={33},
  number={5},
  pages={1255--1262},
  year={2017},
  publisher={IEEE}
}


@article{bescos2018dynaslam,
  title={DynaSLAM: Tracking, mapping, and inpainting in dynamic scenes},
  author={Bescos, Berta and F{\'a}cil, Jos{\'e} M and Civera, Javier and Neira, Jos{\'e}},
  journal={IEEE Robotics and Automation Letters},
  volume={3},
  number={4},
  pages={4076--4083},
  year={2018},
  publisher={IEEE}
}

@article{li2020deepslam,
  title={DeepSLAM: A robust monocular SLAM system with unsupervised deep learning},
  author={Li, Ruihao and Wang, Sen and Gu, Dongbing},
  journal={IEEE Transactions on Industrial Electronics},
  volume={68},
  number={4},
  pages={3577--3587},
  year={2020},
  publisher={IEEE}
}

@incollection{katz2007direct,
  title={Direct visibility of point sets},
  author={Katz, Sagi and Tal, Ayellet and Basri, Ronen},
  booktitle={ACM SIGGRAPH 2007 papers},
  pages={24--es},
  year={2007}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{chen2022overview,
  title={An overview on visual slam: From tradition to semantic},
  author={Chen, Weifeng and Shang, Guangtao and Ji, Aihong and Zhou, Chengjun and Wang, Xiyang and Xu, Chonghui and Li, Zhenxiong and Hu, Kai},
  journal={Remote Sensing},
  volume={14},
  number={13},
  pages={3010},
  year={2022},
  publisher={MDPI}
}

@inproceedings{triggs2000bundle,
  title={Bundle adjustment—a modern synthesis},
  author={Triggs, Bill and McLauchlan, Philip F and Hartley, Richard I and Fitzgibbon, Andrew W},
  booktitle={Vision Algorithms: Theory and Practice: International Workshop on Vision Algorithms Corfu, Greece, September 21--22, 1999 Proceedings},
  pages={298--372},
  year={2000},
  organization={Springer}
}

@article{mur2015orb,
  title={ORB-SLAM: a versatile and accurate monocular SLAM system},
  author={Mur-Artal, Raul and Montiel, Jose Maria Martinez and Tardos, Juan D},
  journal={IEEE transactions on robotics},
  volume={31},
  number={5},
  pages={1147--1163},
  year={2015},
  publisher={IEEE}
}

@article{macario2022comprehensive,
  title={A comprehensive survey of visual slam algorithms},
  author={Macario Barros, Andr{\'e}a and Michel, Maugan and Moline, Yoann and Corre, Gwenol{\'e} and Carrel, Fr{\'e}d{\'e}rick},
  journal={Robotics},
  volume={11},
  number={1},
  pages={24},
  year={2022},
  publisher={MDPI}
}

@article{roldao20223d,
  title={3D semantic scene completion: A survey},
  author={Roldao, Luis and De Charette, Raoul and Verroust-Blondet, Anne},
  journal={International Journal of Computer Vision},
  volume={130},
  number={8},
  pages={1978--2005},
  year={2022},
  publisher={Springer}
}

@inproceedings{huang2023tri,
  title={Tri-perspective view for vision-based 3d semantic occupancy prediction},
  author={Huang, Yuanhui and Zheng, Wenzhao and Zhang, Yunpeng and Zhou, Jie and Lu, Jiwen},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={9223--9232},
  year={2023}
}

@inproceedings{segal2009generalized,
  title={Generalized-icp.},
  author={Segal, Aleksandr and Haehnel, Dirk and Thrun, Sebastian},
  booktitle={Robotics: science and systems},
  volume={2},
  number={4},
  pages={435},
  year={2009},
  organization={Seattle, WA}
}

@inproceedings{park2017colored,
  title={Colored point cloud registration revisited},
  author={Park, Jaesik and Zhou, Qian-Yi and Koltun, Vladlen},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={143--152},
  year={2017}
}

@inproceedings{duan2022pfilter,
  title={PFilter: Building Persistent Maps through Feature Filtering for Fast and Accurate LiDAR-based SLAM},
  author={Duan, Yifan and Peng, Jie and Zhang, Yu and Ji, Jianmin and Zhang, Yanyong},
  booktitle={2022 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={11087--11093},
  year={2022},
  organization={IEEE}
}

@article{tian2023occ3d,
  title={Occ3D: A Large-Scale 3D Occupancy Prediction Benchmark for Autonomous Driving},
  author={Tian, Xiaoyu and Jiang, Tao and Yun, Longfei and Wang, Yue and Wang, Yilun and Zhao, Hang},
  journal={arXiv preprint arXiv:2304.14365},
  year={2023}
}

@inproceedings{caesar2020nuscenes,
  title={nuscenes: A multimodal dataset for autonomous driving},
  author={Caesar, Holger and Bankiti, Varun and Lang, Alex H and Vora, Sourabh and Liong, Venice Erin and Xu, Qiang and Krishnan, Anush and Pan, Yu and Baldan, Giancarlo and Beijbom, Oscar},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={11621--11631},
  year={2020}
}

@article{campos2021orb,
  title={Orb-slam3: An accurate open-source library for visual, visual--inertial, and multimap slam},
  author={Campos, Carlos and Elvira, Richard and Rodr{\'\i}guez, Juan J G{\'o}mez and Montiel, Jos{\'e} MM and Tard{\'o}s, Juan D},
  journal={IEEE Transactions on Robotics},
  volume={37},
  number={6},
  pages={1874--1890},
  year={2021},
  publisher={IEEE}
}

@article{qian20223d,
  title={3D object detection for autonomous driving: A survey},
  author={Qian, Rui and Lai, Xin and Li, Xirong},
  journal={Pattern Recognition},
  volume={130},
  pages={108796},
  year={2022},
  publisher={Elsevier}
}

@article{rist2021semantic,
  title={Semantic scene completion using local deep implicit functions on lidar data},
  author={Rist, Christoph B and Emmerichs, David and Enzweiler, Markus and Gavrila, Dariu M},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={44},
  number={10},
  pages={7205--7218},
  year={2021},
  publisher={IEEE}
}

@incollection{zhong2020semantic,
  title={Semantic point completion network for 3D semantic scene completion},
  author={Zhong, Min and Zeng, Gang},
  booktitle={ECAI 2020},
  pages={2824--2831},
  year={2020},
  publisher={IOS Press}
}

@inproceedings{song2017semantic,
  title={Semantic scene completion from a single depth image},
  author={Song, Shuran and Yu, Fisher and Zeng, Andy and Chang, Angel X and Savva, Manolis and Funkhouser, Thomas},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1746--1754},
  year={2017}
}

@inproceedings{Garbade_Chen_Sawatzky_Gall_2019,  
 title={Two Stream 3D Semantic Scene Completion}, 
 url={http://dx.doi.org/10.1109/cvprw.2019.00055}, 
 DOI={10.1109/cvprw.2019.00055}, 
 booktitle={2019 IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops (CVPRW)}, 
 author={Garbade, Martin and Chen, Yueh-Tung and Sawatzky, Johann and Gall, Juergen}, 
 year={2019}, 
 month={Jun}, 
 language={en-US} 
 }

@inproceedings{li2020attention,
  title={Attention-based multi-modal fusion network for semantic scene completion},
  author={Li, Siqi and Zou, Changqing and Li, Yipeng and Zhao, Xibin and Gao, Yue},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={34},
  number={07},
  pages={11402--11409},
  year={2020}
}

@INPROCEEDINGS{9320345,
  author={Wu, Shun-Cheng and Tateno, Keisuke and Navab, Nassir and Tombari, Federico},
  booktitle={2020 International Conference on 3D Vision (3DV)}, 
  title={SCFusion: Real-time Incremental Scene Reconstruction with Semantic Completion}, 
  year={2020},
  volume={},
  number={},
  pages={801-810},
  doi={10.1109/3DV50981.2020.00090}
}

@inproceedings{cao2022monoscene,
    title={MonoScene: Monocular 3D Semantic Scene Completion}, 
    author={Anh-Quan Cao and Raoul de Charette},
    booktitle={CVPR},
    year={2022}
}

@article{miao2023occdepth,
  title={Occdepth: A depth-aware method for 3d semantic scene completion},
  author={Miao, Ruihang and Liu, Weizhou and Chen, Mingrui and Gong, Zheng and Xu, Weixin and Hu, Chen and Zhou, Shuchang},
  journal={arXiv preprint arXiv:2302.13540},
  year={2023}
}

@inproceedings{engel2014lsd,
  title={LSD-SLAM: Large-scale direct monocular SLAM},
  author={Engel, Jakob and Sch{\"o}ps, Thomas and Cremers, Daniel},
  booktitle={Computer Vision--ECCV 2014: 13th European Conference, Zurich, Switzerland, September 6-12, 2014, Proceedings, Part II 13},
  pages={834--849},
  year={2014},
  organization={Springer}
}

@inproceedings{tateno2017cnn,
  title={Cnn-slam: Real-time dense monocular slam with learned depth prediction},
  author={Tateno, Keisuke and Tombari, Federico and Laina, Iro and Navab, Nassir},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={6243--6252},
  year={2017}
}

@article{teed2021droid,
  title={Droid-slam: Deep visual slam for monocular, stereo, and rgb-d cameras},
  author={Teed, Zachary and Deng, Jia},
  journal={Advances in neural information processing systems},
  volume={34},
  pages={16558--16569},
  year={2021}
}

@inproceedings{sucar2021imap,
  title={iMAP: Implicit mapping and positioning in real-time},
  author={Sucar, Edgar and Liu, Shikun and Ortiz, Joseph and Davison, Andrew J},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={6229--6238},
  year={2021}
}

@inproceedings{zhu2022nice,
  title={Nice-slam: Neural implicit scalable encoding for slam},
  author={Zhu, Zihan and Peng, Songyou and Larsson, Viktor and Xu, Weiwei and Bao, Hujun and Cui, Zhaopeng and Oswald, Martin R and Pollefeys, Marc},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12786--12796},
  year={2022}
}

@inproceedings{ross2022bev,
  title={BEV-SLAM: Building a Globally-Consistent World Map Using Monocular Vision},
  author={Ross, James and Mendez, Oscar and Saha, Avishkar and Johnson, Mark and Bowden, Richard},
  booktitle={2022 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={3830--3836},
  year={2022},
  organization={IEEE}
}

@inproceedings{besl1992method,
  title={Method for registration of 3-D shapes},
  author={Besl, Paul J and McKay, Neil D},
  booktitle={Sensor fusion IV: control paradigms and data structures},
  volume={1611},
  pages={586--606},
  year={1992},
  organization={Spie}
}

@inproceedings{zhang2016degeneracy,
  title={On degeneracy of optimization-based state estimation problems},
  author={Zhang, Ji and Kaess, Michael and Singh, Sanjiv},
  booktitle={2016 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={809--816},
  year={2016},
  organization={IEEE}
}

@inproceedings{iverson1962programming,
  title={A programming language},
  author={Iverson, Kenneth E},
  booktitle={Proceedings of the May 1-3, 1962, spring joint computer conference},
  pages={345--351},
  year={1962}
}

@misc{grupp2017evo,
  title={evo: Python package for the evaluation of odometry and SLAM.},
  author={Grupp, Michael},
  howpublished={\url{https://github.com/MichaelGrupp/evo}},
  year={2017}
}

==> table/map_compare_backup.tex <==
\definecolor{barriercolor}{RGB}{255,0,0}
\definecolor{trafficconecolor}{RGB}{255,165,0}
\definecolor{drivablesurfacecolor}{RGB}{135,206,235}
\definecolor{otherflatcolor}{RGB}{165,42,42}
\definecolor{sidewalkcolor}{RGB}{211,211,211}
\definecolor{terraincolor}{RGB}{153,102,51}
\definecolor{manmadecolor}{RGB}{128,128,128}
\definecolor{vegetationcolor}{RGB}{34,139,34}

\newcolumntype{M}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table*}[]
\centering
\caption{Partial visualization results on Occ3D-nuScenes validation sequences}
\vspace{-1.0em}
\label{map_compare_table}
% \begin{tabular}{|c|M{0.55\columnwidth}|M{0.55\columnwidth}|M{0.55\columnwidth}|}
\begin{tabular}{c M{0.55\columnwidth} M{0.55\columnwidth} M{0.55\columnwidth}}
%\hline
Input Sequence & OCC-VO(ours) & OCC-VO(without \pfilter) & Ground Truth \\ %\hline

% Scene-0012     & 
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_012_pred.png}}\end{minipage} &
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_012_np.png}}\end{minipage} & 
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_012_gt.png}}\end{minipage} \\ \hline

% Scene-0101     & 
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_101_pred.png}}\end{minipage} &
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_101_np.png}}\end{minipage} & 
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_101_gt.png}}\end{minipage} \\ \hline

% Scene-0103     & 
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_103_pred.png}}\end{minipage} &
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_103_np.png}}\end{minipage} & 
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_103_gt.png}}\end{minipage} \\ \hline

Scene-0268     & 
\begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_268_pred.png}}\end{minipage} &
\begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_268_np.png}}\end{minipage} & 
\begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_268_gt.png}}\end{minipage} \\ %\hline

Scene-0269     & 
\begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_269_pred.png}}\end{minipage} &
\begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_269_np.png}}\end{minipage} & 
\begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_269_gt.png}}\end{minipage} \\ %\hline

% Scene-0273     & 
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_273_pred.png}}\end{minipage} &
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_273_np.png}}\end{minipage} & 
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_273_gt.png}}\end{minipage} \\ \hline

Scene-0802     & 
\begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_802_pred.png}}\end{minipage} &
\begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_802_np.png}}\end{minipage} & 
\begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_802_gt.png}}\end{minipage} \\ %\hline

% Scene-0971     & 
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_971_pred.png}}\end{minipage} &
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_971_np.png}}\end{minipage} & 
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_971_gt.png}}\end{minipage} \\ \hline

% Scene-0972     & 
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_972_pred.png}}\end{minipage} &
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_972_np.png}}\end{minipage} & 
% \begin{minipage}[b]{0.55\columnwidth}\raisebox{-.45\height}{\includegraphics[width=\linewidth]{fig/result/scene_972_gt.png}}\end{minipage} \\ \hline

\end{tabular}

\vspace{2pt}

\begin{tabular}{*{16}{@{}l}}
\raisebox{0.25ex}{\colorbox{barriercolor}{\rule{0pt}{1ex}\rule{1ex}{0pt}}} & \,Barrier \hspace{1em} &
\raisebox{0.25ex}{\colorbox{trafficconecolor}{\rule{0pt}{1ex}\rule{1ex}{0pt}}} & \,Traffic cone \hspace{1em} &
\raisebox{0.25ex}{\colorbox{drivablesurfacecolor}{\rule{0pt}{1ex}\rule{1ex}{0pt}}} & \,Driveable surface \hspace{1em} &
\raisebox{0.25ex}{\colorbox{otherflatcolor}{\rule{0pt}{1ex}\rule{1ex}{0pt}}} & \,Other flat \hspace{1em} &
\raisebox{0.25ex}{\colorbox{sidewalkcolor}{\rule{0pt}{1ex}\rule{1ex}{0pt}}} & \,Sidewalk \hspace{1em} &
\raisebox{0.25ex}{\colorbox{terraincolor}{\rule{0pt}{1ex}\rule{1ex}{0pt}}} & \,Terrain \hspace{1em} &
\raisebox{0.25ex}{\colorbox{manmadecolor}{\rule{0pt}{1ex}\rule{1ex}{0pt}}} & \,Manmade \hspace{1em} &
\raisebox{0.25ex}{\colorbox{vegetationcolor}{\rule{0pt}{1ex}\rule{1ex}{0pt}}} & \,Vegetation\\
\end{tabular}
\vspace{-2.0em}
\end{table*}
